DTFD-MIL: Double-Tier Feature Distillation Multiple Instance Learning for Histopathology Whole Slide Image Classification

Multiple instance learning (MIL) has been increasingly used in the classification of histopathology whole slide images (WSIs). However, MIL approaches for this specific classification problem still face unique challenges, particularly those related to small sample cohorts. In these, there are limited number of WSI slides (bags), while the resolution of a single WSI is huge, which leads to a large number of patches (instances) cropped from this slide. To address this issue, we propose to virtually enlarge the number of bags by introducing the concept of pseudo-bags, on which a double-tier MIL framework is built to effectively use the intrinsic features. Besides, we also contribute to deriving the instance probability under the framework of attention-based MIL, and utilize the derivation to help construct and analyze the proposed framework. The proposed method outperforms other latest methods on the CAMELYON-16 by substantially large margins, and is also better in performance on the TCGA lung cancer dataset. The proposed framework is ready to be extended for wider MIL applications. The code is available at: https://github.com/hrzhang1123/DTFD-MIL

==> blank.tex <==

\author{Hongrun Zhang$^{1,5}$, Yanda Meng$^{1}$, Yitian Zhao$^{2}$, Yihong Qiao$^{3}$, Xiaoyun Yang$^{4}$, Sarah Coupland$^{5,6}$ \\ Yalin Zheng$^{1}$\Letter\\ 
$^{1}$Department of Eye and Vision Science, University of Liverpool, Liverpool, United Kingdom\\
$^{2}$Cixi Institute of Biomedical Engineering, Chinese Academy of Sciences, Ningbo, China\\
$^{3}$China Science IntelliCloud Technology Co., Ltd, Shanghai, China \\ 
$^{4}$Remark AI UK Limited, London, United Kingdom \\
$^{5}$Liverpool Ocular Oncology Research Group, University of Liverpool, Liverpool, UK \\
$^{6}$Liverpool Clinical Laboratories, Liverpool University Hospitals NHS Foundation Trust, Liverpool,UK \\
{\tt\small  \{hongrun.zhang,   yanda.meng, S.E.Coupland, yalin.zheng\}@liverpool.ac.uk } 
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
%\and
%Second Author\\
%Institution2\\
%First line of institution2 address\\
%{\tt\small secondauthor@i2.org}
}
